Exploring Phrase-Level Grounding with Text-to-Image Diffusion Model

Recently, diffusion models have increasingly demonstrated their capabilities in vision understanding. By leveraging prompt-based learning to construct sentences, these models have shown proficiency in classification and visual grounding tasks. However, existing approaches primarily showcase their ability to perform sentence-level localization, leaving the potential for leveraging contextual information for phrase-level understanding largely unexplored. In this paper, we utilize Panoptic Narrative Grounding (PNG) as a proxy task to investigate this capability further. PNG aims to segment object instances mentioned by multiple noun phrases within a given narrative text. Specifically, we introduce the DiffPNG framework, a straightforward yet effective approach that fully capitalizes on the diffusion's architecture for segmentation by decomposing the process into a sequence of localization, segmentation, and refinement steps. The framework initially identifies anchor points using cross-attention mechanisms and subsequently performs segmentation with self-attention to achieve zero-shot PNG. Moreover, we introduce a refinement module based on SAM to enhance the quality of the segmentation masks. Our extensive experiments on the PNG dataset demonstrate that DiffPNG achieves strong performance in the zero-shot PNG task setting, conclusively proving the diffusion model's capability for context-aware, phrase-level understanding. Source code is available at \url{https://github.com/nini0919/DiffPNG}.

==> table/tab2.tex <==
\begin{table*}[t]
\centering
\caption{DiffPNG Ablation Experiment.}
\vspace{-10pt}
\begin{tabular}{@{}c|ccccc@{}}
\toprule
Approach & Overall & Singular & Plural & Thing & Stuff \\
\midrule
Random & 15.53 & 15.76 & 13.47 & 11.9 & 20.58 \\
Baseline (Cross) & 30.19 & 30.61 & 26.35 & 26.82 & 34.87 \\
Baseline (Cross) + Self &33.54       & 34.05      & 28.93      & 29.79     &38.74 \\
Baseline + Text + Self + SAM & \textbf{38.8} & \textbf{39.53} & \textbf{32.26} & \textbf{36.59} & \textbf{41.88} \\
\bottomrule
\end{tabular}
\label{tab:weight}
\end{table*}

==> table/tab5.tex <==
\begin{table}[]
\centering
\caption{Different inversion.}
\vspace{-10pt}
    \begin{tabular}{@{}cccccc@{}}
    \toprule
          & overall & singular & plural & thing & stuff \\
          \midrule
    no inversion &       &       &       &       &  \\
    ddim inversion &       &       &       &       &  \\
    null text inversion &       &       &       &       &  \\
    direct inversion &       &       &       &       &  \\
\bottomrule
\end{tabular}
\label{tab:weight}

\end{table}
